Differentiable Neural Architecture Search for Extremely Lightweight Image Super-Resolution

Single Image Super-Resolution (SISR) tasks have achieved significant performance with deep neural networks. However, the large number of parameters in CNN-based met-hods for SISR tasks require heavy computations. Although several efficient SISR models have been recently proposed, most are handcrafted and thus lack flexibility. In this work, we propose a novel differentiable Neural Architecture Search (NAS) approach on both the cell-level and network-level to search for lightweight SISR models. Specifically, the cell-level search space is designed based on an information distillation mechanism, focusing on the combinations of lightweight operations and aiming to build a more lightweight and accurate SR structure. The network-level search space is designed to consider the feature connections among the cells and aims to find which information flow benefits the cell most to boost the performance. Unlike the existing Reinforcement Learning (RL) or Evolutionary Algorithm (EA) based NAS methods for SISR tasks, our search pipeline is fully differentiable, and the lightweight SISR models can be efficiently searched on both the cell-level and network-level jointly on a single GPU. Experiments show that our methods can achieve state-of-the-art performance on the benchmark datasets in terms of PSNR, SSIM, and model complexity with merely 68G Multi-Adds for $\times 2$ and 18G Multi-Adds for $\times 4$ SR tasks.

==> 8.bio.tex <==
\vspace{-2cm}
\begin{IEEEbiography}
    [{\includegraphics[height=1.1in,clip,keepaspectratio]{hanhuang}}]{Han Huang}
received the MS degree from Xidian University, Xi’an, China, in 2021. She has been a
research intern with Tencent AI Lab in 2020. She is currently with Tencent Data Platform, Shenzhen, China. Her research interests include computer vision and  automatic machine learning.
\end{IEEEbiography}

\vspace{-2cm}
\begin{IEEEbiography}
[{\includegraphics[height=1.16in,clip,keepaspectratio]{lishen.jpg}}]
{Li Shen} received his Ph.D. in school of mathematics, South China University of Technology in 2017. He is currently a research scientist at JD Explore Academy, China. Previously, he was a research scientist at Tencent AI Lab, China. His research interests include theory and algorithms for large scale convex/nonconvex/minimax optimization problems, and their applications in statistical machine learning, deep learning, reinforcement learning, and game theory. He is the corresponding author.
\end{IEEEbiography}

\vspace{-2cm}
\begin{IEEEbiography}
[{\includegraphics[width=1in,clip,keepaspectratio]{chaoyanghe.png}}]
{Chaoyang He} is Co-founder and CTO of FedML, Inc., a startup running for a community building open and collaborative AI from anywhere at any scale. His research focuses on distributed/federated machine learning algorithms, systems, and applications. He received his Ph.D. in Computer Science from the University of Southern California, Los Angeles, USA, advised by Salman Avestimehr. Previously, He was an R\&D Team Manager and Principal Software Engineer at Tencent and a Team Leader and Senior Software Engineer at Baidu.
\end{IEEEbiography}


\vspace{-2cm}
\begin{IEEEbiography}
[{\includegraphics[height=1.16in,clip,keepaspectratio]{weishengdong}}]{Weisheng Dong} (Member, IEEE) received the B.S.degree in electronic engineering from the Huazhong University of Science and Technology, Wuhan, China, in 2004, and the Ph.D. degree in circuits and system from Xidian University, Xi’an, China, in 2010. He was a Visiting Student with Microsoft Research Asia, Bejing, China, in 2006. From 2009 to 2010, he was a Research Assistant with the Department of Computing, Hong Kong Polytechnic University, Hong Kong. In 2010, he joined Xidian University, as a Lecturer, and has been a Professor since 2016. He is now with the School of Artificial Intelligence, Xidian University. His research interests include inverse problems in image processing, sparse signal representation, and image compression. He is currently serving as an associate editor of IEEE Transactions on Image Processing and SIAM Journal of Imaging Sciences.
\end{IEEEbiography}

%\vspace{-3cm}
\begin{IEEEbiography}
[{\includegraphics[height=1.16in,clip,keepaspectratio]{WeiLiu.jpg}}]{Wei Liu} (M'14-SM'19) is currently a Distinguished Scientist of Tencent and the Director of Ads Multimedia AI at Tencent Data Platform. Prior to that, he has been a research staff member of IBM T. J. Watson Research Center, USA. Dr. Liu has long been devoted to fundamental research and technology development in core fields of AI, including deep learning, machine learning, computer vision, pattern recognition, information retrieval, big data, etc. To date, he has published extensively in these fields with more than 270 peer-reviewed technical papers, and also issued 23 US patents. He currently serves on the editorial boards of IEEE TPAMI, TNNLS, IEEE Intelligent Systems, and Transactions on Machine Learning Research. He is an Area Chair of top-tier computer science and AI conferences, e.g., NeurIPS, ICML, IEEE CVPR, IEEE ICCV, IJCAI, and AAAI. Dr. Liu is a Fellow of the IEEE, IAPR, AAIA, IMA, RSA, and BCS, and an Elected Member of the ISI.  
\end{IEEEbiography}
